Snippext: Semi-supervised Opinion Mining with Augmented Data

Online services are interested in solutions to opinion mining, which is the problem of extracting aspects, opinions, and sentiments from text. One method to mine opinions is to leverage the recent success of pre-trained language models which can be fine-tuned to obtain high-quality extractions from reviews. However, fine-tuning language models still requires a non-trivial amount of training data. In this paper, we study the problem of how to significantly reduce the amount of labeled training data required in fine-tuning language models for opinion mining. We describe Snippext, an opinion mining system developed over a language model that is fine-tuned through semi-supervised learning with augmented data. A novelty of Snippext is its clever use of a two-prong approach to achieve state-of-the-art (SOTA) performance with little labeled training data through: (1) data augmentation to automatically generate more labeled training data from existing ones, and (2) a semi-supervised learning technique to leverage the massive amount of unlabeled data in addition to the (limited amount of) labeled data. We show with extensive experiments that Snippext performs comparably and can even exceed previous SOTA results on several opinion mining tasks with only half the training data required. Furthermore, it achieves new SOTA results when all training data are leveraged. By comparison to a baseline pipeline, we found that Snippext extracts significantly more fine-grained opinions which enable new opportunities of downstream applications.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> content/augment-old.tex <==
\newcommand{\tfidf}{\ensuremath{\mathsf{TFIDF}}}
\newcommand{\similarity}{\ensuremath{\mathsf{sim}}}
\newcommand{\bert}{\ensuremath{\mathsf{BERT}}}
\newcommand{\aug}{\ensuremath{\text{aug}}}

\section{Data Augmentation} \label{sec:da}
Data augmentation (\da) is a technique to 
automatically 
increase the size of the training data without
using human annotators. DA is shown to be effective for certain tasks in computer vision and NLP.
In computer vision, 
labeled images that are augmented through simple operators such as rotate, crop, pad, flip are shown to be 
effective for training
deep neural networks \cite{perez2017effectiveness,autoaugment}.
In NLP, sentences that are augmented by 
replacing tokens with their corresponding synonyms are shown to be effective for training sentence classifiers~\cite{eda}.
Intuitively, such augmented data
allow the trained model to learn properties 
that remain invariant in the data (e.g., the meaning of a sentence remains unchanged if a token is replaced with its synonym).
\wctan{stopped here}
Inspired by the existing $\da$ operators, we introduce an extended collection of regular $\da$ operators (Section \ref{sec:regularda}) that are suitable for both the tagging and span-classification tasks considered in \snippext.


Training a model over an augmented dataset is not always beneficial since 
the regular $\da$ operators can distort the training examples by too much and 
hurt the performance of the resulting model. 
To avoid this, we introduce $\mixda$ (Section \ref{sec:mixda}), 
a novel technique that restricts \yuliang{reduces?} the distortion introduced by the regular $\da$ operators. 
Essentially, instead of directly using the noisy augmented example,
$\mixda$ computes a convex interpolation
of the original example with the augmented example and use
the interpolation as the training signal.
Therefore, it allows a regular operator to be applied only partially during the training process.
\yuliang{modified.}

%However, as we show later in Section 3.1, the standard set of NLP $\da$ operators can distort the training examples by too much so that they can hurt the performance of the resulting model.To overcome this challenge, we proceed as follows.
%As our first step, we extend the set of the basic operators with new ones
%that are suitable for the tagging and span-classification tasks considered in \snippext.
%(Section \ref{sec:spanda}).
%We also considered the $\mixup$ operator. Unlike the regular $\da$ operators which
%augment a single example at a time, $\mixup$ combines two examples into a new one
%by computing their convex interpolation. 
%While this can be easily done for images, it is unclear how to interpolate text data. 
%Finally, we combine $\mixup$ with the regular operators into a brand-new set of $\da$ operators, $\mixda$,
%which allows a regular operator to be applied only partially (Section \ref{sec:mixda}). 

\subsection{A collection of regular DA operators}\label{sec:regularda}

\zhengjie{I'm not sure whether this argument ``In NLP, data augmentation is mostly used for generating new examples for sentence classification tasks. '' is helpful. }

In NLP, there are some common data augmentation opeartors\cite{eda,xie2019unsupervised} including
%The commonly used operators \cite{eda,xie2019unsupervised} include: 
token replacement (\textbf{TR}), which replaces a token from the example with a new one; 
token insertion (\textbf{INS}), which inserts a token into the example; 
token deletion (\textbf{DEL}), which deletes a token from the example; 
token swap (\textbf{SW}), which swaps two tokens in the example; 
and back translation (\textbf{BT}), 
which translates the example into a different language and then translate it back, e.g., EN $\rightarrow$ FR $\rightarrow$ EN.
%Although being effective for sentence classification, 
%a direct application of these operators over the tagging or span classification tasks could be problematic.
Although these opeartors are very effective for sentence classification, 
a direct application of these operators over the tagging or span classification tasks could be problematic.
\begin{example} \label{ex:regularda}
Let us consider a simple labeled example from the Aspect/Opinion Extraction task:\
\begin{center}
\small
\begin{tabular}{ccccccc}
The & \textbf{food} & was & \textbf{average} & \textbf{at} &\textbf{best} &.\\
O&\textbf{B-AS} & O&\textbf{B-OP}&\textbf{I-OP}&\textbf{I-OP}&O\\
\end{tabular} 
\end{center} 
\textbf{SW} and \textbf{DEL} can move/delete the ``average(B-OP)'' token,
leaving the sequence in an inconsistent state (i.e., I-OP not preceded by B-OP).
\textbf{TR} and \textbf{INS} can change the meaning of tokens and make the original tags invalid, e.g., by replacing ``at'' with ``and'', the correct tags should be ``average (B-OP) and(O) best(B-OP)''. 
Even worse, \textbf{BT} can corrupt the sentence structure since the tagging information is lost during translation, which makes it impossible to obtain the correct tags in the result text.
\end{example}
From the above example, we found that the tags separate the example sequence into two generic types: the 
consecutive subsequences with non-``$\otag$'' tags (or consecutive subsequences represented by a pair of 
indices in span classification tasks), which we call the \textbf{target spans}; 
and the tokens with ``$\otag$'' tags, which we call the \textbf{non-target tokens}. 
In addition, we observed that it is impossible to guarantee the correctness 
of the tagging sequence if we apply $\da$ operators over \textbf{target spans}.
Therefore, we consider only the 4 token-level operators (\textbf{TR}, \textbf{INS}, \textbf{DEL}, and \textbf{SW}) and 
apply them over the \textbf{non-target tokens}. 
To leverage the \textbf{target spans} for $\da$, we introduce a new span-level replacement (\textbf{SPR}) operator, 
which augments the input sequences by replacing a target span 
with a new span of the same type. \yuliang{missing discussion of target spans for span-classification tasks.} Table~\ref{tab:da} summarizes the extended collection of regular $\da$ operator types in \snippext.



\begin{table}[t]
\small
\vspace{-2mm}
\caption{\small Regular Data Augmentation Operator Types.} \vspace{-3mm}
\label{tab:da}
\begin{tabular}{c|p{5cm}} \toprule
\textbf{Operator Type}  &\multicolumn{}{1}{\textbf{Description}}\\\midrule
\textbf{TR} & Replace \textbf{non-target token} with a new token. \\ 
\textbf{INS} & Insert before or after a \textbf{non-target token} with a new token. \\
\textbf{DEL}       & Delete a \textbf{non-target token}. \\ 
\textbf{SW}         & Swap two \textbf{non-target tokens}. \\\midrule
\textbf{SPR}     & Replace a \textbf{target span} with a new span.\\\bottomrule
\end{tabular}
\end{table}


The collection of regular $\da$ operators involves two sampling tasks: First, sampling tokens/spans from the original example to perform the operator\footnote{We also need to sample a token for \textbf{INS} such that the new token will be added after the sampled token.}, which we call pre-sampling; Second, sampling a new token/span to insert or replace the original token/span, which we call post-sampling and it only applies to \textbf{INS}, \textbf{TR}, and \textbf{SPR}. In \snippext, we consider three strategies in pre-sampling and post-sampling tasks.

\begin{itemize}
\item Uniform (pre/post-sampling): This is a commonly used strategy~\cite{eda}, which relies uniform sampling to choose token/span.
\item Importance (pre/post-sampling): This strategy samples tokens/spans with the probability proportional to the importance of the token/span, which is measured by token's TF-IDF value~\cite{xie2019unsupervised} or the span's frequency.
\item Semantic Similarity (post-sampling only): This strategy samples tokens/spans with the probability proportional to its semantic similarity with the original token/span. Here, we measure the semantic similarity by the cosine similarity over token's/span's embeddings\footnote{For token, we use  Word2Vec \cite{word2vec} embeddings; for spans, we use the BERT encoding.}.
\end{itemize}
In practice, we explored different combinations of pre-sampling and post-sampling strategies and report the most effective strategies in Section~\ref{sec:experiment}. 
\xiaolan{Add more details.}

\iffalse

\begin{center}
\begin{tabular}{c|c|c|c} \toprule
& \multicolumn{3}{c}{\textbf{Post-sampling}}  \\\cline{2-4}
\textbf{Pre-sampling}     & Uniform & Importance & Semantic Sim. \\ \hline
Uniform & \textbf{SPR} & \textbf{SPR-FREQ} & \textbf{TR}, \textbf{SPR-SIM}\\ \hline
Importance & - & - & \textbf{TR-TFIDF}\\ \bottomrule
\end{tabular}
\end{center}

\noindent Note that for \textbf{TR}, we do not consider Uniform/Importance strategies during post-sampling since they may introduce too much noise to the augmented example; for \textbf{SPR}, we do not consider Importance strategy during pre-sampling since there 
are normally only a few target spans in one example with similar importance.



For all the operators, we follow the commonly used sampling strategy~\cite{eda}, 
uniform sampling, to select the token/span from the original example to replace/insert/delete/swap. 
For \textbf{TR} and \textbf{SPR}, we consider the following strategies in choosing the new token/span.
\yuliang{TODO: clarify TFIDF}
\begin{itemize}
\item Uniform Sampling \textbf{(TR, SPR)}: Sample tokens/spans uniformly from the vocabulary/training set.
\item Importance \textbf{(TR-TFIDF, SPR-FREQ)}: Sample tokens/spans with the probability that is proportional to the token's/span's frequency in the vocabulary/training set. 
\item Semantic Similarity \textbf{(TR-SIM, SPR-SIM)}: Sample tokens/spans with the probability that is proportional to their semantic similarity with the original span. Here, we measure the semantic similarity by the cosine similarity over tokens'/spans' embeddings\footnote{For token, we use  Word2Vec \cite{word2vec} embeddings; for spans, we use the BERT encoding.}
\end{itemize}
\fi

\subsection{MixDA: augment by interpolating examples} \label{sec:mixda}
Although we carefully select and tailor our collection of regular $\da$ operators, training a model directly over the augmented dataset could be risky: these operators can still
distort the training examples by too much and hurt the performance of the resulting model. 
This is in contrast to the $\da$ operators in images, which are generally noise-free, 
applying the regular $\da$ operators, even when \emph{a single operator is applied only once}, 
can still introduce too much noise. 

\yuliang{add back the example.}
\begin{example}
Suppose we want to augment the following example for classifying the aspect sentiment
of ``Everybody'':
\begin{center}
\underline{Everybody} (+1) was very nice ...
\end{center}
Even after we take into account the target spans, the operators can still generate
examples that can potentially harm the trained model.
\textbf{TR} can replace ``nice'' with a negative/neutral word (e.g., ``poor'', ``okay'')
and change the label from +1 to -1 or 0.
Similarly, \textbf{DEL} can drop ``nice'', \textbf{INS} can insert ``not'' after ``was'',
or \textbf{SPR} can replace ``Everybody'' with ``Nobody'' to distort the sentiment label.
\end{example}

Therefore, 
in \snippext, we introduce a novel technique called $\mixda$ , which combines an example and an augmented example into a new one, to restrict the distortion and resolve this issue. 

$\mixda$ is inspired by and largely follows the $\mixup$ operator \cite{mixup,verma2018manifold} in computer vision. $\mixup$ 
operator is an very effective regularization technique for learning better image representations. Essentially, it
produce new training examples by combining two existing examples through their convex interpolation. Leveraging these combined examples, 
the trained model can therefore makes predictions that
are ``smooth'' in between the two examples. For example, in a binary classification of 
cat and dog images, the model would learn that (1) the ``combination'' of two cats (or dogs) should be
classified as cat (or dog); (2) something ``in between'' a cat and a dog should be given less confidence, i.e., the model should predict both classes with close probability.

Unlike images, the input sequences in NLP are
not continuous and have different length, 
thus we cannot apply the convex interpolation directly 
over the sequences. In \snippext, instead of interpolating 
the input sequences (or their word embeddings), 
we compute the language model's encoding of the two sequences 
and interpolate the encoded sequences. 
A similar idea was considered in computer vision \cite{verma2018manifold}
and shown to be more effective than directly interpolating the inputs.
\xiaolan{more justification?} \yuliang{pls check.}

\smallskip
\noindent \textbf{\textbf{MixUp}$\mathbf{^{NL}}$. }
%\xiaolan{Give it a better name, e.g., \ensuremath{\mathsf{MixUp^+}} or \ensuremath{\mathsf{MixUp^{NLP}}}.}
Let $x_1$ and $x_2$ be two text sequences and $y_1$ and $y_2$ as their one-hot label vectors\footnote{For tagging task, $y_1$ and $y_2$
are sequences of vectors.} respectively.
We assume that both sequences are padded into the same length.
$\mixda$ creates a new sequence $x'$ from $x_1$ and $x_2$ as the follows.
\begin{eqnarray}
\bert(x') &=& \lambda \cdot \bert(x_1) + (1-\lambda) \cdot \bert(x_2) \label{interpolation:x}\\
y' &=& \lambda \cdot y_1 + (1-\lambda) \cdot y_2 \label{interpolation:y}
\end{eqnarray}
where $\bert(x_1)$ and $\bert(x_2)$ are the BERT encoding for $x_1$ and $x_2$, and
$\lambda \in [0, 1]$ is a random variable sampled from a symmetric 
Beta distribution $\text{Beta}(\alpha, \alpha)$ for a hyper-parameter $\alpha$.
Note that we do not actually generate the interpolated sequence $x'$ but
only use the interpolated encoding $\bert(x')$ to carry out the computation
in the task-specific layers of the neural network.
\yuliang{I was thinking whether we should plot the beta distribution here.}

% \smallskip

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.43\textwidth]{content/figs/da3.pdf}
    \caption{\small MixDA: augment by interpolating over the BERT encoding layer.}
    \label{fig:mixda}
\end{figure}
%figs in: https://docs.google.com/presentation/d/1_0OY4F46rvNZ4PeD3R_Ek0ihvj2HBlK0WoORTAgC3AI/edit#slide=id.g63a2bc8436_0_80

Figure~\ref{fig:mixda} illustrates how we apply $\mixda$ during training. 
Given an example $(x, y)$, $\mixda$ trains a model through three main steps:
\begin{itemize}
\item \textbf{Data Augmentation}: $\mixda$ first applies one of the $\da$ operator in Section~\ref{sec:regularda} to obtain $(x_\aug, y_\aug)$. 
\item \textbf{Interpolation}: $\mixda$ then performs the $\mixupnl$ interpolation on the 
pair of input $(x, y)$ and $(x_\aug, y_\aug)$ to obtain $(\bert(x'), y')$. 
Since the labels in the original example are tend to be more precise, we need to ensure 
that the BERT interpolation is more likely to be close to the original example $(x, y)$.
This is done by setting the interpolation parameter $\lambda \leftarrow \max\{1 - \lambda, \lambda\}$.
\item \textbf{Back Propagation}: Finally, $\mixda$ feeds the interpolated encoding $\bert(x')$
to the remaining layers, computes loss over $y'$, and back propagates to update the model.
\end{itemize}

\noindent \textbf{Data Augmentation optimization. } 
In order to further reduce the distortion caused by the $\da$ operator, 
$\mixda$ further optimizes the 1st step, data augmentation, by a careful alignment of the
label sequence $y_\aug$  with $y$. This is done by inserting padding tokens
to both $x$ and $x_\aug$ when the inserting/deleting/replacing of tokens/spans create any misalignment
in the two sequences.
When the two sequences are perfectly aligned, Equation~\ref{interpolation:y}
can be simplified as $y'=y_1$. % \xiaolan{maybe add this paragraph under Data Augmentation step. }

In essence, by interpolating the original sequence with the fully augmented sequence,
$\mixda$ is able to generate a new example that is \emph{partially augmented}, or roughly speaking, augmented by a fraction of $1 - \lambda$ instead of 1. This effectively restricts the distortion introduced by the regular $\da$ operators. Our experiment confirms
that $\mixda$ outperforms regular $\da$ by up to 1.2\% in aspect extraction.
\yuliang{added a number.}

\iffalse
\section{Data Augmentation (old)}
\subsection{Review of basic DA operators} \label{sec:regularda}
We start by reviewing the commonly used $\da$ operators for NLP.
\begin{itemize}
\item \textbf{Token Replacement (TR)}:
Replace a randomly sampled token with a different word.
Commonly used sampling strategies include uniform sampling \cite{eda}
and sampling with probability proportional to the negative TF-IDF of each token \cite{xie2019unsupervised}
(less important tokens are more likely).
There are also multiple strategies for choosing the resulting word:
by similarity (e.g., dictionary, embeddings, etc.) or 
by importance (TF-IDF).
We tried various combinations of strategies and found the following
most effective: given a sequence $S$,
sample a token $s$ w.p. proportional to
$ \max_{s \in S}\{\tfidf(s)\} - \tfidf(s) $
and replace it with a word $w$ sampled from
the $k$ most similar words to $s$
w.p. proportional to $\similarity(s, w)$.
\wctan{I don't understand the prev sentence. why can't we simply consider $ \max_{s \in S}\{\tfidf(s)\}$ since the term is a constant. }
Here $\similarity(s, w)$ is the cosine similarity of the Word2Vec \cite{word2vec}
word embedding of $s$ and $w$ trained on a corpus of in-domain unlabeled text.
We denote this method by $\textbf{TR-TFIDF}$. For comparison, 
we also consider a variant which samples tokens uniformly denoted by simply $\textbf{TR}$.
\item \textbf{Token Insertion (INS)}:
This method inserts a token at a random position of the input sequence.
The position is sampled uniformly and the inserted token is a random similar word
of a random token in the original sequence.
\item \textbf{Token deletion (DEL)}:
This method deletes a random token. Similar to $\textbf{TR}$, the chosen token
can be uniformly sampled or with probability proportional to the negative TF-IDF.
We denote these two variants by $\textbf{DEL}$ and $\textbf{DEL-TFIDF}$ respectively.
\item \textbf{Swap (SW)}: Swap two randomly selected tokens. 
This method swaps two tokens chosen uniformly at random.
\item \textbf{Back Translation (BT)}: Translate the input to a different language and translated back 
(e.g., EN $\rightarrow$ FR $\rightarrow$ EN).
\end{itemize}

Although being effective for sentence classification, 
a direct application of these operators over the tagging or span classification setting could be problematic.
Consider the example of Aspect/Opinion extraction:
\begin{center}
... the food(B-AS) was average(B-OP) at(I-OP) best(I-OP) .
\end{center}
\textbf{SW} and \textbf{DEL} can move/delete the ``average(B-OP)'' token
leaving the sequence in an inconsistent state (i.e., I-OP not preceded by B-OP).
\textbf{TR} and \textbf{INS} can change tokens' meaning in the target span 
invalidating the original tags. For example, replacing ``at'' $\rightarrow$ ``and''
the correct labels should change to ``average(B-OP) and best(B-OP)''.
\textbf{BT} is not even applicable. An EN $\rightarrow$ RU $\rightarrow$ EN
back-translation turns the sentence into ``best food at average''. 
The change of the grammatical structure makes it impossible to track the aspect/opinion spans
in the result text. The same situations occur for span-classification tasks (ASC and pairing).
For example, deleting the word ``food'' would result in a useless example for training.

Based on these observations, we made the following design choice.
We consider only the 4 token-level operators (\textbf{TR}, \textbf{INS}, \textbf{DEL}, and \textbf{SW})
and these operators are applied only to tokens that are not in a \emph{target span}.
Specifically, the target spans for tagging are the consecutive subsequences of non-``$\otag$'' tokens or
the span set $P$ for span-classification. Also, to leverage the target spans for $\da$,
we propose a new \emph{span-level} operator, which we describe next.

\subsection{The span-level DA operators} \label{sec:spanda}
The span-level operator (\textbf{SPR}) augment the input sequences by replacing a target span 
with a new span of the same type. For span-classification tasks, we also change the target span in the span set accordingly.
In the above example, an augmented sequence by the span operator
can be 
\begin{center}
... steak(B-AS) house(I-AS) was average(B-OP) at(I-OP) best(I-OP)
\end{center}
Intuitively, such transformation allows the model to focus more on the sentence structure:
any span is likely to be an aspect if it is followed by a ``was'' and an opinion expression.

Like in the token replacement operator, there are multiple ways of sampling the new span.
We consider 3 variants: 
\begin{itemize}\parskip=0pt
\item \textbf{SPR}: sampling spans from the training set uniformly at random,
\item \textbf{SPR-FREQ}: sampling w.p. proportional to the span's frequency in the training set, and
\item \textbf{SPR-SIM} sampling w.p. proportional to the similarity with the original span.
We measure the similarity of two spans by the cosine of their BERT encoding\footnote{of the ``[CLS]'' token, specifically}.
\end{itemize}

\yuliang{TODO: more intuition, and maybe an example}


\subsection{MixUp: augment by interpolating examples} \label{sec:mixup}
$\mixup$ is another $\da$ operator that we consider.
Unlike the regular operators which augment one example at a time,
$\mixup$ combines two existing examples into a new example as their convex interpolation.
%It can be described as the following simple steps.
Given two examples $(x_1, y_1)$ and $(x_2, y_2)$ where $x_1, x_2$ are two continuous feature vectors
and $y_1, y_2$ are the one-hot label vectors,
\begin{itemize}\parskip=0pt
\item[($\dag$)] Sample $\lambda \in [0, 1]$ from a symmetric 
Beta distribution $\text{Beta}(\alpha, \alpha)$ for a hyper-parameter $\alpha$,
return a new example $(x', y')$ where
\begin{equation}
x' := \lambda x_1 + (1 - \lambda) x_2, \quad y' := \lambda y_1 + (1 - \lambda) y_2 
\end{equation}
\end{itemize}

Intuitively, $\mixup$ introduces these new examples so that the trained model makes predictions that
are ``smooth'' in between the two examples. For example, in a binary classification of 
cat and dog images, the model would learn that (1) the ``combination'' of two cats (or dogs) should be
classified as cat (or dog); (2) something ``in between'' a cat and a dog should be given less confidence,
i.e., the model should predict both classes with close probability.

$\mixup$ is shown to be an effective regularization technique 
for learning better image representations \cite{mixup,verma2018manifold}.
However, it is unclear how to directly apply $\mixup$ in the NLP setting as the input sequences are
not continuous. Our design choice largely follows \cite{verma2018manifold}.
Instead of interpolating the input sequences (or their word embeddings),
we compute the BERT encoding of the two sequences and interpolate the encoded sequences.

Figure \ref{fig:mixup} illustrates how we apply $\mixup$ during training.
The algorithm takes as input two sequences $x_1, x_2$ and computes the encoded sequences $\bert(x_1), \bert(x_2)$.
We then interpolate the two sequences into $\bert(x') := \lambda \bert(x_1) + (1 - \lambda) \bert(x_2) $.
Here $x'$ is the ``interpolated'' sequence. It is not actually generated but we have $\bert(x')$ as its BERT layers' output.
We then compute with the remaining layers, compute the loss (the cross-entropy wrt  
$\lambda y_1 + (1 - \lambda) y_2$) and backpropagate to update both the linear and the BERT layers.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.49\textwidth]{content/mixup.pdf}
    \caption{\small MixUp on the BERT encoding layer}
    \label{fig:mixup}
\end{figure}

\yuliang{TODO: comment on why mixup works for NLP or our setting.}

\subsection{MixedDA: combine regular DA with MixUp} \label{sec:mixda}
The effect of the regular $\da$ operators can be insignificant or even negative
as they still might distort the original sequence by so much that
the resulting sequence becomes too noisy. In the above example,
suppose we want to augment the following example for classifying the aspect sentiment
of ``Everybody'':
\begin{center}
\underline{Everybody} (+1) was very nice ...
\end{center}

Even after we take into account the target spans, the operators can still generate
examples that can potentially harm the trained model.
\textbf{TR} can replace ``nice'' with a negative/neutral word (e.g., ``poor'', ``okay'')
and change the label from +1 to -1 or 0.
Similarly, \textbf{DEL} can drop ``nice'', \textbf{INS} can insert ``not'' after ``was'',
or \textbf{SR} can replace ``Everybody'' with ``Nobody'' to distort the sentiment label.

Unlike the $\da$ operators for images which are generally noise-free,
we observe that the NLP operators can be \emph{too noisy} even when 
\emph{a single operator is applied once}.
So we propose $\mixda$. 
By combing the operator with $\mixup$,
$\mixda$ allows a $\da$ operator to be applied partially. 
For each sequence $x$ with labels $y$ to be augmented, $\mixda$:
\begin{enumerate}\parskip=0pt
\item applies the $\da$ operator to obtain $(x_\aug, y_\aug)$;
\item performs $\mixup$ on the pair of input $(x, y)$ and $(x_\aug, y_\aug)$.
\end{enumerate}

We also adjust the $\mixup$ procedure and each $\da$ as follows.
For $\mixup$, we need to ensure that the interpolation is more likely to be close to the original example $(x, y)$.
This is done by setting the interpolation parameter $\lambda \leftarrow \max\{1 - \lambda, \lambda\}$.
For the regular $\da$, specifically for tagging, 
we need to ensure that the augmented label sequence $y_\aug$ is aligned with $y$.
This is done by a careful implementation that inserts padding tokens
to both $x$ and $x_\aug$ if any misalignment is created when inserting/deleting/replacing
tokens or spans.

In essence, by interpolating the original sequence with the fully augmented sequence,
the resulting example is \emph{partially augmented}, or roughly speaking,
augmented by a fraction of $1 - \lambda$ instead of 1.
In the above example, the interpolation of ``\underline{Everybody} was very nice'' with
``\underline{Nobody} was very nice'' is more likely to be closer to the original sentence
so that the sentiment label is less likely to be distorted.
This is confirmed by our experiment results which
show that $\mixda$ outperforms $\mixup$ and regular $\da$ by up to X\%.

% Finally, we combine $\mixup$ with the regular $\da$ operators.
% distortion
% 
\fi

==> content/intro-old.tex <==
\section{Introduction (OLD)} \label{sec:intro}
\xiaolan{The title says text mining, and the intro starts from online reviews. Maybe we can first say something about the what is text mining and why people conduct text mining. e.g., Many of online services are built upon text data, e.g., wikipedia, tripadvisors. The growth of these online services has brought people great convenience, but also makes it harder and harder to find the right information from the massive amount of unstructured text data. For example, online reviews play an important role in decision-making process, ... At the same time, I feel text mining is way too broad, it can be NER, knowledge base construction, information retrieval, and etc. So, maybe having "review" in the title is OK. }

Online reviews play an important role in our daily decision-making processes,
ranging from buying electronic products, booking a romantic vacation
to housing and even career planning. \yuliang{citations}
While being very useful, most of the time, reading reviews can be 
an overwhelming activity for online users caused by reviews being too long, too many,
or containing too much irrelevant information.
As such, it is a necessity of extracting useful structured information from reviews
so that they can be summarized, indexed, then queried efficiently by the users.


\begin{example}\label{exm:extractor}
Figure \ref{fig:extractor} shows an example of extracting structured data
from hotel reviews. Each extraction is an expression of a customer experience or an opinion of
the form ``$\attr: (\asp, \opi, s)$'' like ``\textbf{Facility}: (\emph{elevator}, \emph{a bit slow}, -1)''. 
The expression consists of two spans of tokens:
an \emph{aspect term} $\asp$ representing the target of the opinion (e.g., ``breakfast''),
an \emph{opinion term} $\opi$ representing the detailed opinion expression 
(e.g., ``not very exciting'', $\bot$ if absent). 
\wctan{can asp be absent?}
In addition, the expression is assigned with a polarity score where
$+1$ means positive, $-1$ means negative and $0$ means neutral. \wctan{so this means it is one of the 3 values or is it a value between -1 and 1?}
Each expression is also assigned
to an \emph{experiential attribute} $\attr$ (e.g., ``food'', ``cleanliness'', ``staff'') 
from a fixed set of 21 hotel attributes that the application considers important.
Such extractions have been used for query processing \cite{opinedb} and
experiential travel search \cite{voyageur} and have a good potential in many more applications.
\yuliang{maybe more examples here.}
\end{example}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.48\textwidth]{content/extractor.pdf}
    \caption{\small{Extractions from a hotel review. \wctan{should add what are teh attributes also since you just described it.}}}
    \label{fig:extractor}
\end{figure}

Depending on the need of the application, the extraction problem can be formulated differently,
ranging from the simple document-level sentiment classification 
\cite{liu2012sentiment,zhang2015character,maas2011learning} to
the more informative Aspect-Based Sentiment Analysis (ABSA) \cite{pontiki2014semeval, pontiki2015semeval} or
Targeted ABSA \cite{sentihood}.
Opinion Mining has been an active line of research for over a decade
with many meaningful extraction tasks proposed (see \cite{liu2012sentiment} for a survey).
Oftentimes, these extraction problems are solved by decomposing into multiple common subtasks
of \emph{sequence tagging}, \emph{span-level classification}, and \emph{sentence-level classification}.
Figure \ref{fig:subtasks} shows an example of decomposing 
the extraction task in Example \ref{exm:extractor} into a tagging subtask and 2 span classification subtasks.
\wctan{but the figure also shows the pairing subtask}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{content/subtasks.pdf}
    \caption{\small{First, the tagging model identifies all aspect (AS) and opinion (OP) spans. 
    Among all candidate pairs of AS-OP spans, the pairing model identifies the correct extractions,
    e.g., (``very clean'', ``room'') is correct but not (``big'', ``staff''). 
    Finally, a classifier decides which attribute that an extracted pair should be assigned to.}}
    \label{fig:subtasks}
\end{figure}

The recent success of transfer learning \cite{bert,spanbert,xlnet} in NLP provides
a simple yet powerful solution for training high-quality models for each subtask.
One simply needs to apply a pre-trained language model like BERT \cite{bert}
and fine-tune it using labeled data of each individual subtask. %\yuliang{can mention huggingface too}
Figure \ref{fig:bert} illustrates an example of fine-tuning BERT for extracting aspect and opinion terms.
It has been shown in \cite{posttrain,auxiliarysentence,opinedb}
that BERT with proper fine-tuning achieved state-of-the-art (SOTA) performance in many extraction subtasks
outperforming the previous customized neural network approaches. \yuliang{too many paper to cite here.}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{content/model_architecture.pdf}
    \caption{\small{Fine-tuning BERT for aspect/opinion term extraction.} \xiaolan{In-domain BERT is not explained until sec 2. Should we add some description?}}
    \label{fig:bert}
\end{figure}


While being very effective, the fine-tuning approach still suffers from a major limiting factor 
as in many deep learning approaches -- it requires a significant
amount of high-quality labeled training data.
Collecting such labeled examples is hard and expensive. %\yuliang{it will be good if there is a paper to cite} 
For example, the SOTA Aspect Term Extraction (AE) model for restaurants is trained on
3,841 sentences labeled by linguistic experts through a nontrivial process \cite{pontiki2014semeval}. \yuliang{check for correctness} \xiaolan{we can also say something about the crowdsourcing tasks, e.g., crowdsourcing process is also expensive and very error prone: at the Figure8 platform, collecting 1k labeled sents may cost \$ xx with xx error rate.}
To make things even worse, 
this expensive labeling process needs to be repeated every time the model needs to be applied to a different domain (say, hotel reviews),
making the SOTA techniques less attractive in practice.
Therefore, it is critically important to reduce the requirement of labeled examples
-- this is the fundamental topic of this paper. We consider the following problem setting:

\begin{problem}
Given an extraction subtask 
(e.g., aspect-opinion extraction, span-level sentiment classification),
can we train / fine-tune a high-quality model (i.e., close to SOTA performance) 
with a small set of training examples (say, 1000 labeled sentences)?
\end{problem}



\subsection{Contributions} \label{sec:contributions}

We consider fine-tuning BERT\footnote{We believe that our methods are 
general enough to be applied to other pre-trained language models.} 
as the starting point and apply an array of optimizations
to reduce the label requirement.

\smallskip
\noindent
\textbf{Data Augmentation. }
Our first optimization is \emph{data augmentation} (\da)
which simply generates new training examples from the existing ones.
It was shown that $\da$ can effectively improve models' quality \cite{autoaugment,xie2019unsupervised,eda}
and reduce the label requirement as a side effect.
For NLP, effective $\da$ operators can be \emph{insert}, \emph{delete}, or \emph{substitute} of tokens.
These operators not just enlarges the training set but in essence, 
allows the models to ``learn'' invariance properties such as 
``the meaning of a sentence stays unchanged if a word is replaced with its synomyms''.
While these operators are shown effective for sentence classification \cite{eda},
they are not ideal for tasks like sequence tagging or span-level classification.
We show examples in Section \ref{sec:da} that these simple operators can distort tags or the meaning of each span
thus hurt the performance of the model with wrong labels.
As our first novel contribute, we propose a new set of $\da$ operators suitable for tagging
and span-level classification. Intuitively, instead of directly applying an operator like token substitution,
the new operators allow the transformation to be applied ``partially'' so that
the resulting sequence can be less distorted.
This is done by a nontrivial adaptation of the $\mixup$ technique \cite{mixup} (Section \ref{sec:da}).

\smallskip
\noindent
\textbf{Semi-Supervised Learning. } 
In our second optimization, we apply the \emph{SOTA semi-supervised learning (SSL)} techniques to
better leverage the massive amount of unlabeled data presented in review corpus.
Among the many SSL algorithms, we consider $\mixmatch$ \cite{mixmatch}
due to its recent great success in computer vision: 
it learns high-accuracy image classifiers when given only a few hundreds of labeled examples.
We review $\mixmatch$ in Section \ref{sec:overview}.
While the result is encouraging, the adaptation of $\mixmatch$ to our setting faces at least two challenges.
\begin{itemize}\parskip=1pt
\item[(1)] $\mixmatch$ requires computing the $\mixup$ convex combination of two input examples. 
While this is easy for images, it is unclear how this can be done for sentences in a meaningful way.
We propose a variant of $\mixup$ that does not combine the input word embeddings,
but combine the BERT encoding of the two sequences instead. 
This variant not only yields a simple yet efficient implementation of $\mixmatch$.
\item[(2)] The quality of the original $\mixmatch$ highly depends on correctly guessing each unlabeled example with
the model prediction on its data-augmented variants. This is problematic in our setting
because of the less effective $\da$ operators and the overall lower model performance (even in the data-rich setting).
We propose a novel method for label guessing: We train the $\mixmatch$ instance together with multiple non-$\mixmatch$ variants
simultaneously in a multitask learning setting -- all the instances share the BERT layers.
We then guess each unlabeled example by averaging
the predictions of all the instances. By doing so, the $\mixmatch$ instance avoids making predictions that are
``consistantly wrong'', yet the non-$\mixmatch$ instances can benefit from the features in the unlabeled data learned via $\mixmatch$.
\end{itemize}
To our knowledge, this is the first work that successfully applies $\mixmatch$ to the NLP settings.

\yuliang{TODO: write about the experiment results}

\yuliang{TODO: add a short summary of the contributions if necessary. Add a structure of the paper.}
In summary, this paper makes the following contributions:
\begin{itemize}
\item 
\end{itemize}

% \smallskip
% \noindent
% \textbf{Multi-task Learning. } 




% The multitask learning framework (or just say we fixed a model?)

% Data Augmentation -- better leverage the few labels

% Semi-Supervised Learning -- also leverage the unlabeled data

% Combining DA and MM in a holistic manner: using MTL!

% Experiments. Outperforming SOTA in the full data setting.
% With only X examples, the model is able to achieve Y F1 scores.



% As a first step, we propose a generic multi-task architecture 
% for extracting useful structured information from online reviews. 
% The framework is general enough to capture both the sequence tagging 
% and span-level classification subtasks in ABSA and \opinedb.


% Previous transfer learning based methods have shown 
% good performance in these tasks. However, these methods suffer from a major limitations:
% they require a significant number of labeled examples (say, a few thousands)
% to train a model of high quality. As such, these methods have only been applied to
% a small number of domains. To address the issue, we propose
% an array of optimizations based on data augmentation and semi-supervised learning.
% Our experiment results show that the combination of these techniques
% help the models achieve state-of-the-art performance while
% only requiring significantly less training examples.

% This paper makes the following contributions:
% \begin{itemize} \parskip=0pt
% \item the architecture
% \item the methods: DA, MixMatch, and combining them
% \item Experiments
% \end{itemize}

